Active Learning of Ordinal Embeddings: A User Study on Football Data

Humans innately measure distance between instances in an unlabeled dataset using an unknown similarity function. Distance metrics can only serve as proxy for similarity in information retrieval of similar instances. Learning a good similarity function from human annotations improves the quality of retrievals. This work uses deep metric learning to learn these user-defined similarity functions from few annotations for a large football trajectory dataset. We adapt an entropy-based active learning method with recent work from triplet mining to collect easy-to-answer but still informative annotations from human participants and use them to train a deep convolutional network that generalizes to unseen samples. Our user study shows that our approach improves the quality of the information retrieval compared to a previous deep metric learning approach that relies on a Siamese network. Specifically, we shed light on the strengths and weaknesses of passive sampling heuristics and active learners alike by analyzing the participants' response efficacy. To this end, we collect accuracy, algorithmic time complexity, the participants' fatigue and time-to-response, qualitative self-assessment and statements, as well as the effects of mixed-expertise annotators and their consistency on model performance and transfer-learning.

==> Draft Active Learning of Ordinal Embeddings Football (TMLR) (arxiv)/backup.tex <==

\subsection{Notions of Similarity}
\label{sec qualitative clustering}

\begin{table}
    \centering
    \begin{tabular}{ |p{2cm}||p{3cm}|p{9cm}|  }
         \hline
         group & notion & example\\
         \hline
         semantic  & team movement & direction (attack or defense); dynamic or static \\
         & ball movement & pass or shot; short or long; at rest \\
         & semantic category & standards (kickoff); situations (pressuring, passing, shot); consistency of category \\
         & team formation & compact; shifting; offensive or defensive \\
         & area & which third; which flank \\
         \hline
         proximity & player and ball & Are there players are near ball? \\
         & directions & direction of ball trajectory\\
         & length of trajectory & \\
         & distances & spatial proximity similar in candidate scenes \\
         \hline
    \end{tabular}
    \caption{Qualitative clustering of responses to questionnaire into \textit{semantic} and \textit{proximity}.}
    \label{table: survey}
\end{table}

% State the overall idea you are trying to demonstrate, test, or prove with a given result
We hypothesize that there are different notions of similarity that may either already be captured by the Euclidean distance metric, or that can be learned from annotations. Recall that we have collected additional meta data on participants notion of similarity using a questionnaire, see Sec.~\ref{sec survey}. This may help distinguish participants that benefit from fine-tuned models and others for whom a generic pre-trained model is sufficient.


% State the analysis that will demonstrate, test, or prove this result.
We test this hypothesis by analysing the participants' responses to the questionnaire and extract two sets of rules, that we categorize as either \textit{semantic} or \textit{proximity}. Semantic rules describe the scenes' semantics whereas proximity rules largely ignore such interpretations. They instead pay closer attention to proximity or only to subsets of trajectories. Then, we assign participants to either group and compare the triplet accuracy of each groups' pre-trained and fine-tuned models.


\begin{figure}[h!]
    \centering
    \includegraphics[width=.6\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_infotuple_unified.pdf}
%        \begin{subfigure}[b]{0.329\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_simple_infotuple_test-rnd.pdf}
%         \caption{\textit{proximity} notion on Rnd.}
%         \label{fig: pre rnd info simple}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.329\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_complex_infotuple_test-rnd.pdf}
%         \caption{\textit{semantic} notion on Rnd.}
%         \label{fig: pre rnd info complex}
%    \end{subfigure}
    \caption{This figure distinguishes two types of similarity, and shows the effectiveness of fine-tuning via InfoTuple active learning in comparison to the pre-trained baseline. Participants are grouped by their qualitative description of similarity, that is either proximity or semantic. Relative gains are greater for more semantically meaningful notions of similarity and the Euclidean similarity captures the proximity notion.}
    \label{fig: pre vs fine info qualitative}
\end{figure}  


% Give the actual result. Refer to the relevant figure and explain how the figure shows this analysis result.
We show the extracted groups in Table~\ref{table: survey} and each groups' triplet accuracy in Fig.~\ref{fig: pre vs fine info qualitative}. We assign participants to either group if they describe multiple of its notions or provide examples that match it. The resulting \textit{proximity} group contains 7 participants and the \textit{semantic} group the remaining 10. We excluded one participant that did not describe their notion. It is noteworthy that intra-rater consistency is not predictive of either group assignment. We report triplet accuracy in Fig.~\ref{fig: pre vs fine info qualitative}. Fine-tuning increases the semantic groups' triplet accuracy from $72.43\%$ of the pre-trained Siamese network to $76.54$\%, whereas the proximity notion leads to a decrease from $68.57$\% to  $66.77$\%.


% Restate the overall idea and tie the result back into the overall idea.
About a third of participants apparently does not profit from additional annotations. On the other hand, participants that analyse the scenes on a deeper semantic level can benefit. For them, fine-tuning can outperform the Siamese baseline, because the Euclidean similarity metric does not adequately capture these more complex similarity functions.










\subsection{Noisy Oracles Affect Learning}
\label{sec: consistency}

% State the overall idea you are trying to demonstrate, test, or prove with a given result
The consistency of replies has an influence on the networks ability to learn user specific similarity functions. A lower consistency is harder to train with, and a pre-trained network performs better on test data than a fine-tuned one. More consistent annotations, however, enable fine-tuning. The InfoTuple active learner benefits from more consistent annotations. 

% State the analysis that will demonstrate, test, or prove this result.
We compare the triplet accuracy for the pre-trained model with all fine-tuned models for each user. We again use the users' self-annotated test sets \textit{Rnd} and compare the accuracy. Additionally, we split the participants into groups of lower and higher consistency. For each group, we compare the pre-trained model with one trained using the InfoTuple active learner to test fine-tuning with more consistent annotations.

% Give the actual result. Refer to the relevant figure and explain how the figure shows this analysis result.
Fig.~\ref{fig: pre vs fine} shows triplet accuracy, ordered by participants' consistency (from low to high). It compares the pre-trained model (horizontal bar) with any fine-tuned model (violin plots).
We show the effect of consistency on the InfoTuple algorithm in Fig.~\ref{fig: pre vs fine info}. For annotators with low consistency, the pre-trained network often performs similar or even better than the finetuned variant. The pre-trained model is a strong baseline for inconsistent annotators. Fig.~\ref{fig: pre rnd info cons} shows that consistent annotations allow the active learner to learn a similar or better model than the pre-trained baseline, with 74\% for the finetuned case vs 69.2\% pre-trained on the test set.

% Restate the overall idea and tie the result back into the overall idea.
Generally, if the pre-trained network is already performing well on a test set, the fine-tuning with inconsistent data tends to decrease test triplet accuracy. It depends on the consistency of the similarity function used for annotations if fine-tuning is beneficial. For consistent participants, i.e., self-assessed experts, better user-specific similarity functions can be learned.



\begin{figure}[h!]
    \centering
        %\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_test-rnd.pdf}
    \caption{The effectiveness of all fine-tuning variants (violin plot) in comparison to the pre-trained Siamese network (horizontal bar) shows the impact of inconsistent oracles and a performance ceiling for the relatively noisy train and test data.}
    \label{fig: pre vs fine}
\end{figure}  



Furthermore, with InfoTuple as the AL sampler, we see strong increases in triplet accuracy over the pre-trained baseline (see Fig.~\ref{fig: pre vs fine info}). The most consistent $\frac{2}{3}$ participants lead to more stable learning and higher triplet accuracy due to their more consistent replies (see Fig.~\ref{fig: pre rnd info cons}). 

\begin{figure}[h!]
    \centering
        \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_least_consistent_infotuple_test-rnd.pdf}
         \caption{Least consistent $\frac{1}{3}$ on Rnd.}
         \label{fig: pre rnd info}
    \end{subfigure}
    \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_consistent_infotuple_test-rnd.pdf}
         \caption{Most consistent $\frac{2}{3}$ on Rnd.}
         \label{fig: pre rnd info cons}
    \end{subfigure}
    \caption{This figure shows the effectiveness of fine-tuning via InfoTuple active learning in comparison to the pre-trained baseline for different levels of consistency. Participants are grouped according to their consistency, into a least consistent third and the most consistent two thirds. Relative gains are greater for more consistent replies.}
    \label{fig: pre vs fine info}
\end{figure}  






\subsection{Larger Cluster of Similarity Functions}
\label{appdx big cluster}

We selected four participants with high inter-rater reliability and repeated the experiments from Sec.~\ref{sec: clusters}. While there is still a mean increase in triplet accuracy of $0.7\%$ to $1.7\%$, it is less stable between the cluster members, and the extended warm-up data can also lead to decreases in performance, e.g., for $p12$ and $p5$ on the NN test data, see Fig.~\ref{fig: big cluster}.

\begin{figure}[h!]
    \centering
     %   \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth, keepaspectratio]{plots/userstudy_big_cluster_rnd.pdf}
         %\caption{Test on Rnd.}
         %\label{fig: big cluster rnd}
    %\end{subfigure}
    %\begin{subfigure}[b]{0.329\textwidth}
    %     \centering
    %     \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_big_cluster_nn.pdf}
    %     \caption{Test on NN.}
    %     \label{fig: big cluster nn}
    %\end{subfigure}
    \caption{The effectiveness of combining more participants' annotations shows less homogeneous improvements in triplet accuracy.}
    \label{fig: big cluster}
\end{figure}  


==> Draft Active Learning of Ordinal Embeddings Football (TMLR) (arxiv)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> backup.tex <==

\subsection{Notions of Similarity}
\label{sec qualitative clustering}

\begin{table}
    \centering
    \begin{tabular}{ |p{2cm}||p{3cm}|p{9cm}|  }
         \hline
         group & notion & example\\
         \hline
         semantic  & team movement & direction (attack or defense); dynamic or static \\
         & ball movement & pass or shot; short or long; at rest \\
         & semantic category & standards (kickoff); situations (pressuring, passing, shot); consistency of category \\
         & team formation & compact; shifting; offensive or defensive \\
         & area & which third; which flank \\
         \hline
         proximity & player and ball & Are there players are near ball? \\
         & directions & direction of ball trajectory\\
         & length of trajectory & \\
         & distances & spatial proximity similar in candidate scenes \\
         \hline
    \end{tabular}
    \caption{Qualitative clustering of responses to questionnaire into \textit{semantic} and \textit{proximity}.}
    \label{table: survey}
\end{table}

% State the overall idea you are trying to demonstrate, test, or prove with a given result
We hypothesize that there are different notions of similarity that may either already be captured by the Euclidean distance metric, or that can be learned from annotations. Recall that we have collected additional meta data on participants notion of similarity using a questionnaire, see Sec.~\ref{sec survey}. This may help distinguish participants that benefit from fine-tuned models and others for whom a generic pre-trained model is sufficient.


% State the analysis that will demonstrate, test, or prove this result.
We test this hypothesis by analysing the participants' responses to the questionnaire and extract two sets of rules, that we categorize as either \textit{semantic} or \textit{proximity}. Semantic rules describe the scenes' semantics whereas proximity rules largely ignore such interpretations. They instead pay closer attention to proximity or only to subsets of trajectories. Then, we assign participants to either group and compare the triplet accuracy of each groups' pre-trained and fine-tuned models.


\begin{figure}[h!]
    \centering
    \includegraphics[width=.6\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_infotuple_unified.pdf}
%        \begin{subfigure}[b]{0.329\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_simple_infotuple_test-rnd.pdf}
%         \caption{\textit{proximity} notion on Rnd.}
%         \label{fig: pre rnd info simple}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.329\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_complex_infotuple_test-rnd.pdf}
%         \caption{\textit{semantic} notion on Rnd.}
%         \label{fig: pre rnd info complex}
%    \end{subfigure}
    \caption{This figure distinguishes two types of similarity, and shows the effectiveness of fine-tuning via InfoTuple active learning in comparison to the pre-trained baseline. Participants are grouped by their qualitative description of similarity, that is either proximity or semantic. Relative gains are greater for more semantically meaningful notions of similarity and the Euclidean similarity captures the proximity notion.}
    \label{fig: pre vs fine info qualitative}
\end{figure}  


% Give the actual result. Refer to the relevant figure and explain how the figure shows this analysis result.
We show the extracted groups in Table~\ref{table: survey} and each groups' triplet accuracy in Fig.~\ref{fig: pre vs fine info qualitative}. We assign participants to either group if they describe multiple of its notions or provide examples that match it. The resulting \textit{proximity} group contains 7 participants and the \textit{semantic} group the remaining 10. We excluded one participant that did not describe their notion. It is noteworthy that intra-rater consistency is not predictive of either group assignment. We report triplet accuracy in Fig.~\ref{fig: pre vs fine info qualitative}. Fine-tuning increases the semantic groups' triplet accuracy from $72.43\%$ of the pre-trained Siamese network to $76.54$\%, whereas the proximity notion leads to a decrease from $68.57$\% to  $66.77$\%.


% Restate the overall idea and tie the result back into the overall idea.
About a third of participants apparently does not profit from additional annotations. On the other hand, participants that analyse the scenes on a deeper semantic level can benefit. For them, fine-tuning can outperform the Siamese baseline, because the Euclidean similarity metric does not adequately capture these more complex similarity functions.










\subsection{Noisy Oracles Affect Learning}
\label{sec: consistency}

% State the overall idea you are trying to demonstrate, test, or prove with a given result
The consistency of replies has an influence on the networks ability to learn user specific similarity functions. A lower consistency is harder to train with, and a pre-trained network performs better on test data than a fine-tuned one. More consistent annotations, however, enable fine-tuning. The InfoTuple active learner benefits from more consistent annotations. 

% State the analysis that will demonstrate, test, or prove this result.
We compare the triplet accuracy for the pre-trained model with all fine-tuned models for each user. We again use the users' self-annotated test sets \textit{Rnd} and compare the accuracy. Additionally, we split the participants into groups of lower and higher consistency. For each group, we compare the pre-trained model with one trained using the InfoTuple active learner to test fine-tuning with more consistent annotations.

% Give the actual result. Refer to the relevant figure and explain how the figure shows this analysis result.
Fig.~\ref{fig: pre vs fine} shows triplet accuracy, ordered by participants' consistency (from low to high). It compares the pre-trained model (horizontal bar) with any fine-tuned model (violin plots).
We show the effect of consistency on the InfoTuple algorithm in Fig.~\ref{fig: pre vs fine info}. For annotators with low consistency, the pre-trained network often performs similar or even better than the finetuned variant. The pre-trained model is a strong baseline for inconsistent annotators. Fig.~\ref{fig: pre rnd info cons} shows that consistent annotations allow the active learner to learn a similar or better model than the pre-trained baseline, with 74\% for the finetuned case vs 69.2\% pre-trained on the test set.

% Restate the overall idea and tie the result back into the overall idea.
Generally, if the pre-trained network is already performing well on a test set, the fine-tuning with inconsistent data tends to decrease test triplet accuracy. It depends on the consistency of the similarity function used for annotations if fine-tuning is beneficial. For consistent participants, i.e., self-assessed experts, better user-specific similarity functions can be learned.



\begin{figure}[h!]
    \centering
        %\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_test-rnd.pdf}
    \caption{The effectiveness of all fine-tuning variants (violin plot) in comparison to the pre-trained Siamese network (horizontal bar) shows the impact of inconsistent oracles and a performance ceiling for the relatively noisy train and test data.}
    \label{fig: pre vs fine}
\end{figure}  



Furthermore, with InfoTuple as the AL sampler, we see strong increases in triplet accuracy over the pre-trained baseline (see Fig.~\ref{fig: pre vs fine info}). The most consistent $\frac{2}{3}$ participants lead to more stable learning and higher triplet accuracy due to their more consistent replies (see Fig.~\ref{fig: pre rnd info cons}). 

\begin{figure}[h!]
    \centering
        \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_least_consistent_infotuple_test-rnd.pdf}
         \caption{Least consistent $\frac{1}{3}$ on Rnd.}
         \label{fig: pre rnd info}
    \end{subfigure}
    \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_pre-vs-fine_consistent_infotuple_test-rnd.pdf}
         \caption{Most consistent $\frac{2}{3}$ on Rnd.}
         \label{fig: pre rnd info cons}
    \end{subfigure}
    \caption{This figure shows the effectiveness of fine-tuning via InfoTuple active learning in comparison to the pre-trained baseline for different levels of consistency. Participants are grouped according to their consistency, into a least consistent third and the most consistent two thirds. Relative gains are greater for more consistent replies.}
    \label{fig: pre vs fine info}
\end{figure}  






\subsection{Larger Cluster of Similarity Functions}
\label{appdx big cluster}

We selected four participants with high inter-rater reliability and repeated the experiments from Sec.~\ref{sec: clusters}. While there is still a mean increase in triplet accuracy of $0.7\%$ to $1.7\%$, it is less stable between the cluster members, and the extended warm-up data can also lead to decreases in performance, e.g., for $p12$ and $p5$ on the NN test data, see Fig.~\ref{fig: big cluster}.

\begin{figure}[h!]
    \centering
     %   \begin{subfigure}[b]{0.329\textwidth}
         \centering
         \includegraphics[width=0.6\textwidth, keepaspectratio]{plots/userstudy_big_cluster_rnd.pdf}
         %\caption{Test on Rnd.}
         %\label{fig: big cluster rnd}
    %\end{subfigure}
    %\begin{subfigure}[b]{0.329\textwidth}
    %     \centering
    %     \includegraphics[width=1.\textwidth, keepaspectratio]{plots/userstudy_big_cluster_nn.pdf}
    %     \caption{Test on NN.}
    %     \label{fig: big cluster nn}
    %\end{subfigure}
    \caption{The effectiveness of combining more participants' annotations shows less homogeneous improvements in triplet accuracy.}
    \label{fig: big cluster}
\end{figure}  

